Preference Learning from Physics-Based Feedback: Tuning Language Models to Design BCC/B2 Superalloys

We apply preference learning to the task of language model-guided design of novel structural alloys. In contrast to prior work that focuses on generating stable inorganic crystals, our approach targets the synthesizeability of a specific structural class: BCC/B2 superalloys, an underexplored family of materials with potential applications in extreme environments. Using three open-weight models (LLaMA-3.1, Gemma-2, and OLMo-2), we demonstrate that language models can be optimized for multiple design objectives using a single, unified reward signal through Direct Preference Optimization (DPO). Unlike prior approaches that rely on heuristic or human-in-the-loop feedback (costly), our reward signal is derived from thermodynamic phase calculations, offering a scientifically grounded criterion for model tuning. To our knowledge, this is the first demonstration of preference-tuning a language model using physics-grounded feedback for structural alloy design. The resulting framework is general and extensible, providing a path forward for intelligent design-space exploration across a range of physical science domains.

==> full_result_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[h]
\centering
\footnotesize
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Model}}                                     & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Median \\ reward\end{tabular}}}} & \multicolumn{2}{c}{\textbf{Passes basic tests}}                                                                              & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% unique \\ pairs\end{tabular}}}} & \multicolumn{3}{c}{\textbf{SFT duplicates}}                                                                                                           & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}ANOVA\\ Pair vs.\\ vol $p$\end{tabular}}}} \\ \cmidrule(lr){3-4} \cmidrule(lr){6-8}
                                                                    & \multicolumn{1}{c}{}                                                                                   & \multicolumn{1}{c}{\textbf{\% pass}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Median \\ reward\end{tabular}}} & \multicolumn{1}{c}{}                                                                                     & \multicolumn{1}{c}{\textbf{BCC}} & \multicolumn{1}{c}{\textbf{B2}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Pair/\\ vol\end{tabular}}} & \multicolumn{1}{c}{}                                                                                             \\ \midrule
SFT training data                                                   & -1.063                                                                                                 & 0.141                                & -0.011                                                                                & 0.986                                                                                                    & 1.000                            & 1.000                           & 1.000                                                                            & 0.700                                                                                                            \\ \midrule
Llama SFT                                                           & -1.074                                                                                                 & 0.162                                & -0.010                                                                                & 0.873                                                                                                    & 0.998                            & 0.999                           & 0.004                                                                            & 0.459                                                                                                            \\
Llama DPO                                                           & -1.033                                                                                                 & 0.206                                & -0.016                                                                                & 0.962                                                                                                    & 1.000                            & 0.997                           & 0.003                                                                            & 0.006                                                                                                            \\
OLMo SFT                                                            & -1.066                                                                                                 & 0.157                                & -0.010                                                                                & 0.861                                                                                                    & 0.995                            & 0.996                           & 0.003                                                                            & 0.542                                                                                                            \\
OLMo DPO                                                            & -11.00                                                                                                 & 0.109                                & -0.014                                                                                & 0.872                                                                                                    & 0.992                            & 0.995                           & 0.008                                                                            & 0.183                                                                                                            \\ \midrule
GPT-o3 few-shot                                                     & -1.008                                                                                                 & 0.218                                & -0.003                                                                                & 0.281                                                                                                    & 0.581                            & 0.230                           & 0.000                                                                            & 0.000                                                                                                            \\
GPT-o3 one-shot                                                     & -11.04                                                                                                 & 0.000                                & -                                                                                     & 0.135                                                                                                    & 0.000                            & 0.001                           & 0.000                                                                            & 0.052                                                                                                            \\
GPT-4.1 few-shot                                                    & -0.003                                                                                                 & 0.575                                & -0.001                                                                                & 0.173                                                                                                    & 0.807                            & 0.252                           & 0.001                                                                            & 0.000                                                                                                            \\
GPT-4.1 one-shot                                                    & -1.059                                                                                                 & 0.000                                & -                                                                                     & 0.100                                                                                                    & 0.000                            & 0.039                           & 0.000                                                                            & 0.151                                                                                                            \\
\begin{tabular}[c]{@{}l@{}}GPT-4.1 few-shot\\ (guided)\end{tabular} & -0.000                                                                                                 & 0.802                                & -0.000                                                                                & 0.020                                                                                                    & 1.000                            & 1.000                           & 0.000                                                                            & 0.000                                                                                                            \\
\begin{tabular}[c]{@{}l@{}}GPT-4.1 one-shot\\ (guided)\end{tabular} & -11.02                                                                                                 & 0.004                                & -0.016                                                                                & 0.102                                                                                                    & 0.998                            & 0.998                           & 0.000                                                                            & 0.001                                                                                                            \\
Gemini few-shot                                                     & -0.066                                                                                                 & 0.513                                & -0.002                                                                                & 0.614                                                                                                    & 0.343                            & 0.605                           & 0.001                                                                            & 0.000                                                                                                            \\
Gemini one-shot                                                     & -11.00                                                                                                 & 0.077                                & -0.002                                                                                & 0.875                                                                                                    & 0.005                            & 0.097                           & 0.000                                                                            & 0.065                                                                                                            \\ \midrule
Random search                                                       & -1112                                                                                                  & 0.009                                & -0.017                                                                                & 0.999                                                                                                    & 0.002                            & 0.066                           & 0.000                                                                            & 0.142                                                                                                            \\ \bottomrule
\end{tabular}

\caption{Full table of model results, including rows omitted from table \ref{tab:summary_table} for brevity.}

\label{tab:full_summary_table}

\end{table*}

==> main_result_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Model}}                                     & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Median \\ reward\end{tabular}}}} & \multicolumn{2}{c}{\textbf{Passes basic tests}}                                                                              & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% unique \\ pairs\end{tabular}}}} & \multicolumn{3}{c}{\textbf{SFT duplicates}}                                                                                                           & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}ANOVA\\ pair vs.\\ vol\% $p$\end{tabular}}}} \\ \cmidrule(lr){3-4} \cmidrule(lr){6-8}
                                                                    & \multicolumn{1}{c}{}                                                                                   & \multicolumn{1}{c}{\textbf{\% pass}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Median \\ reward\end{tabular}}} & \multicolumn{1}{c}{}                                                                                     & \multicolumn{1}{c}{\textbf{BCC}} & \multicolumn{1}{c}{\textbf{B2}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Pair/\\ vol\%\end{tabular}}} & \multicolumn{1}{c}{}                                                                                             \\ \midrule
SFT training sample                                                 & -1.063                                                                                                 & 0.141                                & -0.011                                                                                & 0.986                                                                                                    & 1.000                            & 1.000                           & 1.000                                                                            & 0.700                                                                                                            \\ \midrule
Llama SFT                                                           & -1.074                                                                                                 & 0.162                                & -0.010                                                                                & 0.873                                                                                                    & 0.998                            & 0.999                           & 0.004                                                                            & 0.459                                                                                                            \\
Llama DPO                                                           & -1.033$^{*}$                                                                                                 & 0.206                                & -0.016                                                                                & 0.962                                                                                                    & 1.000                            & 0.997                           & 0.003                                                                            & 0.006                                                                                                            \\
OLMo SFT                                                            & -1.066                                                                                                 & 0.157                                & -0.010                                                                                & 0.861                                                                                                    & 0.995                            & 0.996                           & 0.003                                                                            & 0.542                                                                                                            \\
OLMo DPO                                                             & -11.00$^{*}$                                                                                                 & 0.109                                & -0.014                                                                                & 0.872                                                                                                    & 0.992                            & 0.995                           & 0.008                                                                            & 0.183                                                                                                            \\ \midrule
GPT-4.1 few-shot                                                    & -0.003                                                                                                 & 0.575                                & -0.001                                                                                & 0.173                                                                                                    & 0.807                            & 0.252                           & 0.001                                                                            & 0.000                                                                                                            \\
\begin{tabular}[c]{@{}l@{}}GPT-4.1 few-shot\\ (guided)\end{tabular} & -0.000                                                                                                 & 0.802                                & -0.000                                                                                & 0.020                                                                                                    & 1.000                            & 1.000                           & 0.000                                                                            & 0.000                                                                                                            \\
Gemini few-shot                                                     & -0.066                                                                                                 & 0.513                                & -0.002                                                                                & 0.614                                                                                                    & 0.343                            & 0.605                           & 0.001                                                                            & 0.000                                                                                                            \\ \midrule
Random search                                                       & -1112                                                                                                  & 0.009                                & -0.017                                                                                & 0.999                                                                                                    & 0.002                            & 0.066                           & 0.000                                                                            & 0.142                                                                                                            \\ \bottomrule
\end{tabular}

\caption{Overall summary of SFT, DPO and prompting results. Reward closer to 0 indicates higher quality. Higher \% unique pairs indicates more diverse output. Low-performing models omitted for brevity (full results in Appendix). $^{*}$ indicates significant difference from corresponding SFT model ($p<.05$), per independent t-test.}

\label{tab:summary_table}

\end{table*}

==> topk_table.tex <==
\begin{table*}[h]
\centering
\footnotesize
\begin{tabular}{@{}lcrcrcrcr@{}}
\toprule
\multirow{2}{*}{\textbf{Rank}} & \multicolumn{2}{c}{\textbf{GPT-4.1 few-shot}}         & \multicolumn{2}{c}{\textbf{Gemini-2.5 few-shot}}      & \multicolumn{2}{c}{\textbf{Llama DPO}}                & \multicolumn{2}{c}{\textbf{Llama SFT}}                \\ \cmidrule(l){2-9} 
                               & \textbf{Elements} & \multicolumn{1}{c}{\textbf{Freq}} & \textbf{Elements} & \multicolumn{1}{c}{\textbf{Freq}} & \textbf{Elements} & \multicolumn{1}{c}{\textbf{Freq}} & \textbf{Elements} & \multicolumn{1}{c}{\textbf{Freq}} \\ \midrule
\textbf{1}                     & \{Mo, Nb\}        & 0.500                             & \{Mo, Nb\}        & 0.145                             & \{Nb, Mo, Ti\}    & 0.072                             & \{Cr, Ti, V\}     & 0.041                             \\
\textbf{2}                     & \{W, Nb\}         & 0.382                             & \{W, Mo, Nb\}     & 0.136                             & \{Nb, W, Ti\}     & 0.048                             & \{W, Ti, V\}      & 0.038                             \\
\textbf{3}                     & \{W, Mo, Nb\}     & 0.105                             & \{W, Nb\}         & 0.088                             & \{W, Mo, Nb\}     & 0.048                             & \{Nb, Ti, V\}     & 0.037                             \\
\textbf{4}                     & \{W, Mo, Cr\}     & 0.008                             & \{W, Ta, Nb\}     & 0.073                             & \{W, Mo, Ti\}     & 0.046                             & \{Mo, Ti, V\}     & 0.036                             \\
\textbf{5}                     & \{Nb, V\}         & 0.001                             & \{W, Mo, Cr\}     & 0.062                             & \{Mo, Cr\}        & 0.040                             & \{W, Nb, V\}      & 0.033                             \\ \bottomrule
\end{tabular}

\caption{Top 5 most frequent BCC element combinations generated by each model. }

\label{tab:topk_table}

\end{table*}
